CODEC: Complex Document and Entity Collection

CODEC is a document and entity ranking benchmark that focuses on complex research topics. We target essay-style information needs of social science researchers, i.e. "How has the UK's Open Banking Regulation benefited Challenger Banks?". CODEC includes 42 topics developed by researchers and a new focused web corpus with semantic annotations including entity links. This resource includes expert judgments on 17,509 documents and entities (416.9 per topic) from diverse automatic and interactive manual runs. The manual runs include 387 query reformulations, providing data for query performance prediction and automatic rewriting evaluation. CODEC includes analysis of state-of-the-art systems, including dense retrieval and neural re-ranking. The results show the topics are challenging with headroom for document and entity ranking improvement. Query expansion with entity information shows significant gains in document ranking, demonstrating the resource's value for evaluating and improving entity-oriented search. We also show that the manual query reformulations significantly improve document ranking and entity ranking performance. Overall, CODEC provides challenging research topics to support the development and evaluation of entity-centric search methods.

==> tables/completeness.tex <==
\begin{table}[]
\caption{Average measure of system judgment completeness at different run depths. }
\label{tab:complete}
\begin{tabular}{l|r|r|r|}
\cline{2-4}
                                                & \multicolumn{1}{l|}{\textbf{Judged@5}} & \multicolumn{1}{l|}{\textbf{Judged@10}} & \multicolumn{1}{l|}{\textbf{Judged@20}} \\ \hline
\multicolumn{1}{|l|}{\textbf{Document Runs}} & 83.3\%                                 & 77.9\%                                  & 70.2\%                                  \\ \hline
\multicolumn{1}{|l|}{\textbf{Entity Runs}}   & 85.3\%                                 & 78.3\%                                  & 69.1\%                                  \\ \hline
\end{tabular}
\end{table}

==> tables/document_reformulations.tex <==

\begin{table}[h]
\caption{BM25+RM3 document ranking performance across (1) original query and (2) query reformulations. \iain{better names}}
\label{tab:document-reform}
\begin{tabular}{l|r|r|r|}
\cline{2-4}
\cellcolor[HTML]{FFFFFF}                & \multicolumn{1}{l|}{\textbf{MAP}} & \multicolumn{1}{l|}{\textbf{NDCG@10}} & \multicolumn{1}{l|}{\textbf{Recall@1000}} \\ \hline
\multicolumn{1}{|l|}{\textbf{BM25+RM3}} & 0.223                             & 0.389                                 & 0.795                                     \\ \hline
\multicolumn{1}{|l|}{\textbf{Best-Ref}} & 0.270                             & \textbf{0.392}                        & 0.859                                     \\ \hline
\multicolumn{1}{|l|}{\textbf{Ref-QE}}   & \textbf{0.229}                    & 0.374                                 & \textbf{0.861}                            \\ \hline
\end{tabular}
\end{table}

==> tables/entity_reformulations.tex <==
\begin{table}[h]
\caption{BM25+RM3 entity ranking performance across (1) original query and (2) query reformulations.}
\label{tab:entity-reform}
\begin{tabular}{l|r|r|r|}
\cline{2-4}
\cellcolor[HTML]{FFFFFF}                & \multicolumn{1}{l|}{\textbf{MAP}} & \multicolumn{1}{l|}{\textbf{NDCG@20}} & \multicolumn{1}{l|}{\textbf{Recall@1000}} \\ \hline
\multicolumn{1}{|l|}{\textbf{BM25+RM3}} & 0.196                             & 0.489                                 & 0.656                                     \\ \hline
\multicolumn{1}{|l|}{\textbf{Best-Ref}} & 0.235                             & 0.535                                 & 0.691                                     \\ \hline
\multicolumn{1}{|l|}{\textbf{Ref-QE}}   & 0.243                             & \textbf{0.585}                        & \textbf{0.739}                            \\ \hline
\end{tabular}
\end{table}

==> tables/judgments_breakdown.tex <==

\begin{table}[]
\caption{Judgment distribution by Initial Runs vs. Search.}
\label{tab:judgments-breakdow}
\begin{tabular}{l|r|r|}
\cline{2-3}
                                                & \multicolumn{1}{l|}{\textbf{Initial Runs}} & \multicolumn{1}{l|}{\textbf{Topic Exploration}} \\ \hline
\multicolumn{1}{|l|}{\textbf{Document Ranking}} & 1,896                                      & 3,234                                           \\ \hline
\multicolumn{1}{|l|}{\textbf{Entity Ranking}}   & 2,172                                      & 8,067                                           \\ \hline
\multicolumn{1}{|l|}{\textbf{TOTAL}}            & \textbf{4,068}                             & \textbf{11,301}                                 \\ \hline
\end{tabular}
\end{table}

==> tables/topics_table.tex <==

% \begin{table}[]
% \caption{Example \COMETS topic: economics-1.}
% \label{tab:topic-overview}
% \begin{tabular}{cl}
% \textbf{Domain}    & Economics                                                                                                                                         \\
% \textbf{Query}     & How   has the UK's Open Banking Regulation benefited challenger banks?                                                                                                                                                                                                                                              \\
% \textbf{Narrative} & \begin{tabular}[c]{@{}l@{}}UK’s Open Banking regulation, which has parallels to the EU’s second payment service directive (PSD2), went live in January 2018. This piece of legislation “will require banks to open their payments infrastructure and customer data assets to third parties”. As a result, banks no longer have a monopoly on user data if clients grant permission. 

% Challenger banks are small, recently created retail banks that compete directly with the longer-established banks in the UK. Specifically, seeking market share from the "big four" UK retail banks (Barclays, HSBC, Lloyds Banking Group, and NatWest Group). The banks distinguish themselves from the historic banks by modern financial technology practices, such as online-only operations, that avoid the costs and complexities of traditional banking. The largest UK-operating challenger banks include Atom Bank, Revolut, Starling, N26, and Tide.

% Relevant documents and entities will discuss how challenger banks have used open banking to develop new products or capture market share from traditional retail banks in the UK.\end{tabular}
% \end{tabular}
% \end{table}
